PolyOCR-Venus: Unified OCR Foundation Models for Text-Centric Visual Intelligence

Optical Character Recognition (OCR) is evolving from plain-text transcription toward general visual intelligence, requiring models to recognize, localize, and reason over textual information in complex visual environments. However, existing OCR systems often excel at only some tasks and struggle to balance recognition, parsing, and reasoning across scenarios. In this report, we present PolyOCR, a family of unified OCR foundation models of varying scales. PolyOCR combines a shared instruction-following framework with a large-scale data engine that converts heterogeneous visual resources into quality-verified OCR supervision. We introduce Competence-Guided Policy Optimization, which combines verifier-based Group Relative Policy Optimization with on-policy distillation through sample-wise routing based on teacher reliability and the teacher--student competence gap. We also introduce OCRBench v2.1, our revision of OCRBench v2 with manually verified annotation corrections and task-aligned scoring metrics. Extensive experiments across OCRBench v2.1, CC-OCR, in-house KIE Benchmark, OmniDocBench v1.6 and MDPBench demonstrate that PolyOCR achieves state-of-the-art or highly competitive performance.

==> readme.tex <==
# Antu-α: Unified Visual Understanding & Generation Framework
paper: [url](url)
## Core Technical Breakthroughs

- ### Unified Visual Understanding & Generation Architecture
	Introduces a shared representation space for vision-language tasks, replacing traditional CLIP+Diffusion pipelines. The architecture leverages **learnable multiscale-queries** that dynamically integrate multimodal signals, enabling seamless end-to-end sequence prediction for text→image→editing workflows. This approach effectively addresses the quality limitations of discrete token-based methods. Our Antu-α achieves the unification of generation and understanding, with an average understanding score of 69.7 on the OpenCompass leaderboard, surpassing DeepSeek-VL2 (66.4). At the same time, it maintains strong generation capabilities, achieving a generation score of 61.9 on the GenEval benchmark, outperforming SDXL (0.55).


- ### Multi-Scale Learnable Query Token
	Employs a novel mechanism to establish feature correlations across resolutions of 4×/8×/16×. By introducing **hierarchical tokens**, the model resolves cross-scale inconsistencies in super-resolution and editing tasks. 

- ### Cross-Scale Consistency Loss
  A **cross-scale consistency loss** is applied, leveraging explicit gradient constraints to enhance high-resolution reconstruction quality by more than 2dB PSNR (validated at native resolution).

- ### Connector Module
	Facilitates dynamic alignment of features between frozen MLLM and trainable Diffusion models, achieves semantic alignment for text-to-pixel generation while also ensuring local-global coherence in edits.

- ### AGI-Capable System
	Supports complex chained operations, such as "generate castle → add sunset → adjust perspective," with a swift response time of under 1 second (benchmarked with RTX 4090). The system is designed to handle instruction-driven generation-editing and is synchronized with ChatGPT-4o(aligned with the industry milestone of March 2025).


## Why It Matters

Antu's unified architecture overcomes fundamental limitations of conventional approaches:

| Conventional Methods | Antu's Advantages |
|----------------------|------------------|
| **Modular Pipelines**<br>(CLIP/SigLIP + Diffusion Models) | **End-to-End Unified Model**<br>Seamless understanding-generation integration |
| **Discrete Token AR**<br>(Limited visual grounding) | **Continuous Token Space**<br>Native support for fine-grained visual concepts |
| **Fixed-Resolution Processing**<br>(Artifacts in upscaling) | **Multi-Scale Adaptation**<br>Consistent quality across resolutions |
| **Separate Editing Workflows**<br>(Manual alignment required) | **Dialog-Driven Control**<br>Natural language guided pixel-level editing |
| **Understanding Bottlenecks**<br>(Visual-semantic mismatch) | **Joint Representation Learning**<br>Mutually enhanced comprehension and generation |

## Open Collaboration
We're open-sourcing Antu-α to accelerate progress toward AGI, featuring:
�� Full model weights & test code  
�� Modular architecture for easy extension  
�� Comprehensive benchmarks (vs GPT-4V, SDXL, etc.)

*"The simultaneous release of ChatGPT-4's image generation in March 2025 confirms our vision of unified multimodal AI as the next paradigm."*  

## Empowering Multimodal Interaction with Antu


![效果图](./figures/Ming_unify_usecases.png)
**Antu-α** acts as a unified model for multimodal understanding, extending beyond traditional NLP tasks and multimodal comprehension to enable interactive multimodal generation. This includes capabilities such as image generation, image editing, and style transfer.

## Model Structure

![结构图](./figures/Ming_unify_structure.png)

**Antu-α** is a unified multimodal model designed for both image understanding and high-fidelity image generation. It achieves this by compressing image representations into continuous visual tokens, which are processed alongside discrete text tokens using a scaled auto-regressive Transformer. The generation capability is powered by an externally trained diffusion model (SANA), conditioned on tokens produced by the Transformer.
## Example Usage
- ###Dependencies and Installation
#### System Requirements
- **Python:** >= 3.8
- **PyTorch:** >= 2.4.1+cu12.2 (CUDA 12.2 compatible)

#### Installation

To set up the environment, use pip to install the following dependencies:

```bash
pip install torch==2.4.1 torchvision==0.16.2 torchaudio==2.4.0 tensorflow==2.13.1 numpy==1.24.4 pandas==2.0.1 scipy==1.10.1 scikit-learn==1.3.2 h5py==3.10.0 transformers==4.46.3 diffusers==0.33.0 datasets==2.15.0 sentence-transformers==3.2.1 tokenizers==0.20.3 safetensors==0.4.1 accelerate==0.33.0 deepspeed==0.16.0 bitsandbytes==0.39.0 flash-attn==2.6.3 peft==0.12.0
```

- ### Usage Guided
Below is an example of how to load and use the model:
```python
from transformers import AutoModel, AutoTokenizer

Load the model and tokenizer
model_name = "your-username/your-model-name"
tokenizer = AutoTokenizer.from_pretrained(model_name)
model = AutoModel.from_pretrained(model_name)

Example input
image_file = None
prompt = "Produce image: a smiling man with dark hair sits on a wooden bench wearing a black shirt, khaki pants, and a black belt he accessorizes with a silver and white watch"
generate_prefix = "Production done: <image>" 

Process outputs
print(outputs)
```
For more advanced usage, such as fine-tuning or generating images, refer to the documentation.




## Acknowledgments

The project is currently in its early stages. While some preliminary results have been promising, substantial progress is needed to achieve seamless integration of understanding and generation. Both the code and models require further refinement and optimization, which is why we have chosen to open-source the project. We invite contributions from the community to help enhance and develop it collaboratively. If you have any suggestions or identify issues within the code, please contribute via Pull Requests. Thank you for your support and interest!

## Contact Information

Please submit a GitHub issue if you want help or have issues using Ming.

## License

Ming is licensed under [the MIT License](https://github.com/inclusionAI/Ming/blob/master/LICENCE).



==> sec/7_future.tex <==
7

\section{Future Work}
\enlargethispage{2\baselineskip}
The successful validation of the DeFakerOne paradigm provides a robust starting point for next-generation digital forensics. However, moving toward a universal, intelligent, and highly generalized forensic infrastructure presents several significant challenges. We outline three critical avenues for future research:

\begin{itemize}
\item \textbf{Scalable Foundation Models and Data Engineering}: Our immediate goal is to evolve DeFakerOne from a standalone model into a foundational infrastructure that supports diverse industrial and academic applications. As demonstrated in this study, the simple accumulation of homogeneous data is insufficient to achieve qualitative leaps in model performance. The key challenge lies in developing high-efficiency data pipelines capable of generating high-fidelity, diverse, and representative forensic data at scale. Furthermore, we aim to explore architectural innovations that enhance model generalization in "in-the-wild" environments, where real-world perturbations and unseen forgery patterns remain highly unpredictable.

\item \textbf{Agentic Paradigms for Expert Knowledge Injection}: We intend to advance the integration of expert knowledge through agentic forensic paradigms, specifically by addressing the dichotomy between outcome injection and process injection. While outcome injection is a generalizable approach, it is increasingly limited by the difficulty of obtaining high-quality expert labels. Process injection—such as the construction of Chain-of-Thought (CoT) data—is a promising but immature solution, currently hampered by content homogenization, high reliance on manual design, and poor knowledge transferability. We posit that the future of forensic intelligence lies in leveraging authentic, low-ambiguity ground-truth data in tandem with agentic tools to move beyond static detection toward sophisticated, evidence-based reasoning.

\item \textbf{A Unified Paradigm for Multi-Modal and Physical-Digital Forensics}:
Beyond the current scope of image-level FIDL, we aim to establish a truly unified forensic paradigm. \\
\textbf{Cross-Modal Integration}: Future work will extend the framework to encompass video and audio authentication, creating a cohesive system for multi-modal integrity verification. \\
\textbf{Physical-Digital Synthesis}: We seek to bridge the gap between digital forgery detection and physical anti-spoofing (e.g., mask, replay, and print attacks). Although these attacks differ in their origin, they share fundamental visual forensic traits, such as local trace anomalies, boundary artifacts, and semantic inconsistencies. By incorporating physical contextual metadata—such as device hardware, sensor noise signatures, and environmental factors—we aim to develop a universal forensic foundation. Designing a framework that bridges the physical and digital divide represents the ultimate frontier in artificial intelligence-driven forensics.
\end{itemize}

==> tab/tab_1_benchmarks.tex <==
% \begin{table}
%   \caption{Image-level detection Performance comparison on benchmarks. All results are averaged.}
%   \label{tab:1_seg}
%   \renewcommand{\arraystretch}{0.95} % 将行间距缩小为原来的 0.85 倍
%   \resizebox{0.975\textwidth}{!}{
%   \begin{tabular}{lccccccccccccccc}
%     \toprule
%         % 第一行表头
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{10}{c}{\textbf{Small Vision Models}} & \multicolumn{5}{c}{\textbf{FIDL-domain MLLMs}} \\
    
%         \cmidrule(lr){2-12} \cmidrule(lr){13-16}
        
%         & DTD & FFDN & Trufor & Mesorch & CDFA & Effort & AIDE & DRCT & DDA & Mirror & ForensicMOE & FakeVLM & Veritas & Ivy-xDetector & \modelbase \\
%         \midrule
%         \multicolumn{16}{c}{\textbf{DeepFake (AUC)}} \\
%         FF-c23~\citep{rossler2019faceforensics++} & 21.2 & 73.4 & 53.9 & 49.5 & 94.2 & 92.5 & - & 66.7 & 60.7 & 65.1 & 47.7 & 83.4 & 4.9 & 71.7 & \textbf{99.4} \\
%         FF-c40~\citep{rossler2019faceforensics++} & 20.8 & 79.1 & 49.2 & 49.8 & 79.7 & 80.4 & - & 59.2 & 50.7 & - & 64.9 & 68.8 & 4.4 & 83.1 & \textbf{84.7} \\
%         FF-DF~\citep{rossler2019faceforensics++} & 49.8 & 40.7 & 62.1 & 62.4 & 99.1 & 99.0 & - & 78.8 & 63.0 & - & 46.0 & 63.9 & 3.1 & 73.4 & \textbf{99.8} \\
%         FF-F2F~\citep{rossler2019faceforensics++} & 50.0 & 43.8 & 53.8 & 50.1 & 93.8 & 92.0 & - & 59.3 & 60.1 & - & 36.4 & 60.1 & 3.9 & 67.3 & \textbf{99.2} \\
%         FF-FS~\citep{rossler2019faceforensics++} & 50.2 & 42.6 & 47.0 & 39.3 & 96.5 & 97.2 & - & 76.5 & 57.2 & - & 43.1 & 63.3 & 3.3 & 68.7 & \textbf{99.5} \\
%         FF-NT~\citep{rossler2019faceforensics++} & 49.9 & 49.7 & 52.8 & 46.2 & 87.4 & 81.8 & - & 52.5 & 62.5 & - & 34.9 & 61.7 & 2.8 & 66.6 & \textbf{98.8} \\
%         CDFv1~\citep{li2020celeb} & 38.1 & 54.8 & 54.8 & 48.6 & 91.5 & 90.7 & - & 43.1 & 57.8 & - & 19.9 & 72.2 & 7.8 & 53.0 & \textbf{99.9} \\
%         CDFv2~\citep{li2020celeb} & 34.2 & 61.0 & 55.0 & 53.9 & 91.4 & 88.2 & - & 48.7 & 55.6 & - & 16.2 & 81.9 & 7.9 & 53.6 & \textbf{99.9} \\
%         DFD~\citep{dolhansky2020dfd} & 12.4 & 74.3 & 63.2 & 62.5 & 93.2 & 92.2 & - & 77.4 & 61.1 & - & 81.9 & 88.9 & 7.4 & 77.9 & \textbf{98.7} \\
%         DFDC~\citep{dolhansky2019deepfake} & 47.9 & 47.7 & 51.8 & 50.7 & 84.2 & 82.2 & - & 61.2 & 56.3 & - & 30.6 & 60.1 & 4.5 & 84.2 & \textbf{85.2} \\
%         DFDCP~\citep{dolhansky2019deepfake} & 23.0 & 57.3 & 52.0 & 54.7 & 93.3 & 90.9 & - & 65.7 & 64.9 & - & 16.3 & 84.7 & 5.5 & 90.7 & \textbf{91.0} \\
%         Fsh~\citep{li2019faceshifter} & 50.0 & 43.1 & 54.00 & 52.5 & 77.7 & 88.9 & - & 61.6 & 55.9 & - & 41.2 & 44.6 & 2.3 & 67.3 & \textbf{92.5} \\
%         %UADFV~\citep{li2018uadfv} & - & - & 0.6851 & 0.4412  & - & - & - & - & - & - & 46.6 & 68.2 & 7.1 & 39.3 & - \\
%         % DFo & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         WDF~\citep{zi2020wilddeepfake} & 35.6 & 63.9 & 56.2 & 60.9 & 84.0 & 85.9 & - & 63.4 & 58.9 & - & 21.1 & 63.9 & 6.3 & 82.1 & \textbf{93.0} \\
%         % FFIW & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         %DF40~\citep{yan2024df40} & - & - & 0.5550 & 0.5211 & - & - & - & - & - & - & 56.2 & 76.2 & 7.4 & 71.0 & - \\
%         ScaleDF~\citep{scaledf} & 22.4 & 73.7 & 44.2 & 53.4 & 76.0 & 83.2 & - & 74.6 & 85.0 & - & 55.8 & 73.5 & 81.0 & 82.9 & \textbf{98.6} \\
%         MFFI~\citep{miao2025mffi} & 46.1 & 55.2 & 51.0 & 55.8 & 76.5 & 78.6 & - & - & - & - & 58.1 & 62.6 & 59.2 & 87.4 & \textbf{96.1} \\
%         Avg & 40.7 & 60.2 & 53.8 & 52.6 & 87.9 & 88.2 & - & - & - & - & 45.3 & 69.3 & 12.9 & 72.4 & \textbf{95.6} \\
%         \midrule
%         \multicolumn{16}{c}{\textbf{AIGC (Accuracy)}} \\
%         ForenSynths~\citep{forensyn} & 48.1 & 57.3 & 57.6 & 57.3 & 49.8 & 74.8 & - & 68.6 & 84.7 & - & 71.5 & 71.3 & 69.5 & 77.0 & \textbf{77.2} \\
%         DiffusionForensics~\citep{diffusion_detection} & 21.8 & 55.2 & 51.4 & 55.1 & 59.7 & 71.2 & - & 72.9 & 87.5 & - & 70.9 & 74.9 & 66.5 & 93.5 & \textbf{99.5} \\
%         GenImage~\citep{genimage} & 43.8 & 55.1 & 53.4 & 55.0 & 59.0 & 90.5 & - & 87.8 & 89.4 & - & 94.3 & 99.0 & 80.9 & 96.3 & \textbf{99.7} \\
%         %CommunityForensics~\citep{CommunityForensics} & 30.9 & 35.3 & - & - & - & - & - & 80.2 & 95.9 & - & 89.5 & 92.1 & 89.1 & 94.6 & 34.04 \\
%         Chameleon~\citep{aide} & 36.7 & 37.9 & 41.2 & 37.8 & 55.2 & 63.1 & - & 51.6 & 84.1 & - & 58.9 & 62.9 & 59.6 & 73.2 & \textbf{84.7} \\
%         Fakeinversion~\citep{fakeinversion} & 83.8 & 38.4 & 36.7 & 38.3 & 42.3 & 84.6 & - & 52.4 & 89.2 & - & 81.2 & 70.0 & 57.6 & 66.7 & \textbf{91.8} \\
%         BFree-Online~\citep{bfree} & 36.6 & 67.8 & 60.7 & 67.8 & 38.3 & 55.9 & - & 71.0 & 92.9 & - & 32.9 & 78.6 & 55.2 & 65.5 & 65.7 \\
%         SynthWildx~\citep{SynthWildx} & 51.8 & 43.8 & 45.7 & 43.8 & 41.1 & 57.0 & - & 69.0 & 92.2 & - & 30.2 & 80.2 & 83.2 & 81.9 & 80.1 \\
%         %DRCT-2M~\citep{drct} & - & - & - & - & - & - & - & - & - & - & 65.1 & 77.6 & 63.3 & 78.2 & - \\
%         EvalGEN~\citep{evalgen} & 24.7 & 40.2 & 17.6 & 40.2 & 33.2 & 35.8 & - & 77.7 & 96.9 & - & 18.9 & 92.1 & 90.4 & 93.2 & \textbf{96.4} \\
%         HydraFake~\citep{veritas} & 54.6 & 49.6 & 51.1 & 49.5 & 69.3 & 62.3 & - & 62.7 & 76.5 & - & 60.4 & 77.8 & 87.2 & 71.7 & \textbf{92.8} \\
%         Avg & 44.7 & 49.5 & 46.1 & 49.4 & 49.7 & 66.1 & - & 68.1 & - & - & 49.7 & 79.7 & 73.0 & 81.3 & \textbf{87.5} \\
%         \midrule
%         \multicolumn{16}{c}{\textbf{Doc (Accuracy)}} \\
%         DocTamper\_FCD~\citep{doctamper} & 73.2 & 73.1 & 68.4 & 64.2 & 52.3 & 60.1 & - & 77.0 & 24.6 & - & 38.9 & 1.9 & 39.4 & 25.3 & \textbf{92.8} \\
%         DocTamper\_SCD~\citep{doctamper} & 69.8 & 58.7 & 67.7 & 53.9 & 39.8 & 26.7 & - & 71.8 & 33.4 & - & 24.6 & 1.0 & 31.2 & 25.1 & \textbf{99.8} \\
%         DocTamper\_TestingSet~\citep{doctamper} & 64.3 & 57.8 & - & - & - & - & - & 66.8 & 31.8 & - & 29.8 & 29.5 & 39.0 & 33.9 & \textbf{99.6} \\
%         TextForensicsReasoning~\citep{textshield} & 43.0 & 51.3 & - & - & - & - & - & 52.2 & 64.3 & - & 46.9 & 52.6 & 52.0 & 54.6 & \textbf{99.6} \\
%         Tampered IC13~\citep{wang2022tpic} & 75.3 & 61.9 & - & - & - & - & - & 48.9 & 29.7 & - & 30.5 & 25.3 & 38.2 & 22.8 & 54.9 \\
%         OSTF~\citep{ostf} & 60.3 & 47.0 & - & - & - & - & - & 57.1 & 60.1 & - & 57.9 & 57.0 & 56.8 & 58.0 & \textbf{74.9} \\
%         RTM~\citep{luo2025rtm} & 45.1 & 51.6 & - & - & - & - & - & 63.0 & 37.3 & - & 33.6 & 32.5 & 42.3 & 33.7 & \textbf{90.0} \\
%         RIFLC~\citep{rific} & 70.5 & 58.1 & - & - & - & - & - & 87.7 & 13.6 & - & 1.7 & 0.9 & 30.7 & 8.9 & \textbf{70.0} \\
%         Avg & - & - & - & - & - & - & - & - & - & - & 33.0 & 25.1 & 41.2 & 32.9 & \textbf{85.2} \\
%         \midrule
%         \multicolumn{16}{c}{\textbf{Nature (AUC)}} \\
%         CASIAv1~\citep{CASIA_2013} & 46.8 & 52.5 & - & - & - & - & - & 52.7 & 53.7 & - & 7.7 & 4.2 & 3.2 & 45.8 & \textbf{96.3} \\
%         COVERAGE~\citep{Coverage_2016} & 51.5 & 40.5 & - & - & - & - & - & 52.9 & 48.3 & - & 50.6 & 50.0 & 0.4 & 55.5 & \textbf{75.9} \\
%         Columbia~\citep{Columbia_2006} & 62.3 & 2.20 & - & - & - & - & - & 48.2 & 32.4 & - & 81.7 & 52.6 & 2.5 & 87.6 & \textbf{87.7} \\
%         NIST16~\citep{NIST16_2019} & 56.0 & 38.7 & - & - & - & - & - & 66.7 & 66.6 & - & 3.9 & 58.7 & 1.2 & 55.4 & \textbf{85.1} \\
%         CocoGlide~\citep{trufor2023} & 51.9 & 29.6 & - & - & - & - & - & 72.3 & 68.4 & - & 19.2 & 66.0 & 3.3 & 65.3 & \textbf{76.0} \\
%         Autosplice~\citep{jia2023autosplice} & 42.9 & 34.3 & - & - & - & - & - & 75.5 & 78.0 & - & 37.4 & 67.2 & 4.0 & 40.8 & \textbf{99.9} \\
%         IMD2020~\citep{IMD20_2020} & 35.9 & 75.3 & - & - & - & - & - & 56.5 & 55.4 & - & 5.9 & 67.2 & 4.0 & 47.8 & \textbf{78.0} \\
%         OpenSDI~\citep{opensdi} & 35.2 & 42.5 & - & - & - & - & - & 84.9 & 90.3 & - & 5.0 & 73.5 & 1.9 & 69.5 & \textbf{98.6} \\
%         DSO-1~\citep{dso-1} & 71.0 & 35.0 & - & - & - & - & - & 53.6 & 56.4 & - & 23.2 & 60.5 & 0.5 & 15.1 & \textbf{82.4} \\
%         % DSO-1 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         DEFACTO-12k~\citep{defacto_2019} & 55.1 & 37.8 & - & - & - & - & - & 55.3 & 55.7 & - & 1.7 & 50.0 & 0.9 & 30.9 & \textbf{78.3} \\
%         Avg & - & - & - & - & - & - & - & - & - & - & 23.6 & 55.0 & 2.2 & 51.4 & \textbf{85.8} \\
%   \bottomrule
%   \end{tabular}
% }
% \end{table}






% \begin{table}[]
% \centering
% \begin{tabular}{cccccccc}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{DeepFake} & \multicolumn{2}{c}{Document} & \multicolumn{2}{c}{Nature} & \multirow{2}{*}{Average} \\
%                   & xxx           & xxx          & xxx           & xxx          & xxx          & xxx         &                          \\ \hline
% DTD               &               &              &               &              &              &             &                          \\
% Mesorch           &               &              &               &              &              &             &                          \\
% LEGION            &               &              &               &              &              &             &                          \\
% FakeShield        &               &              &               &              &              &             &                          \\
% DeFakerOne     &               &              &               &              &              &             &                          \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[t]
  \centering
  \caption{Image-level detection performance comparison on benchmarks. All results are averaged.}
  \label{tab:1_seg}
  \renewcommand{\arraystretch}{0.95}
  \resizebox{0.975\textwidth}{!}{
  \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} 
    & \multicolumn{8}{c}{\textbf{Vision Models}} 
    & \multicolumn{4}{c}{\textbf{MLLMs}} \\
    \cmidrule(lr){2-9} \cmidrule(lr){10-13}
    & DTD & FFDN & Trufor & Mesorch & CDFA & Effort & DRCT & ForensicMOE 
    & FakeVLM & Veritas & Ivy-xDetector & \modelbase \\
    \midrule

    \multicolumn{13}{c}{\textbf{DeepFake (AUC)}} \\
    FF-c23~\citep{rossler2019faceforensics++} & 21.2 & 73.4 & 53.9 & 49.5 & \underline{94.2} & 92.5 & 66.7 & 47.7 & 83.4 & 4.9 & 71.7 & \textbf{99.4} \\
    FF-c40~\citep{rossler2019faceforensics++} & 20.8 & 79.1 & 49.2 & 49.8 & 79.7 & 80.4 & 59.2 & 64.9 & 68.8 & 4.4 & \underline{83.1} & \textbf{84.7} \\
    FF-DF~\citep{rossler2019faceforensics++} & 49.8 & 40.7 & 62.1 & 62.4 & \underline{99.1} & 99.0 & 78.8 & 46.0 & 63.9 & 3.1 & 73.4 & \textbf{99.8} \\
    FF-F2F~\citep{rossler2019faceforensics++} & 50.0 & 43.8 & 53.8 & 50.1 & \underline{93.8} & 92.0 & 59.3 & 36.4 & 60.1 & 3.9 & 67.3 & \textbf{99.2} \\
    FF-FS~\citep{rossler2019faceforensics++} & 50.2 & 42.6 & 47.0 & 39.3 & 96.5 & \underline{97.2} & 76.5 & 43.1 & 63.3 & 3.3 & 68.7 & \textbf{99.5} \\
    FF-NT~\citep{rossler2019faceforensics++} & 49.9 & 49.7 & 52.8 & 46.2 & \underline{87.4} & 81.8 & 52.5 & 34.9 & 61.7 & 2.8 & 66.6 & \textbf{98.8} \\
    CDFv1~\citep{li2020celeb} & 38.1 & 54.8 & 54.8 & 48.6 & 91.5 & \underline{90.7} & 43.1 & 19.9 & 72.2 & 7.8 & 53.0 & \textbf{99.9} \\
    CDFv2~\citep{li2020celeb} & 34.2 & 61.0 & 55.0 & 53.9 & \underline{91.4} & 88.2 & 48.7 & 16.2 & 81.9 & 7.9 & 53.6 & \textbf{99.9} \\
    DFD~\citep{dolhansky2020dfd} & 12.4 & 74.3 & 63.2 & 62.5 & \underline{93.2} & 92.2 & 77.4 & 81.9 & 88.9 & 7.4 & 77.9 & \textbf{98.7} \\
    DFDC~\citep{dolhansky2019deepfake} & 47.9 & 47.7 & 51.8 & 50.7 & \underline{84.2} & 82.2 & 61.2 & 30.6 & 60.1 & 4.5 & \underline{84.2} & \textbf{85.2} \\
    DFDCP~\citep{dolhansky2019deepfake} & 23.0 & 57.3 & 52.0 & 54.7 & \textbf{93.3} & 90.9 & 65.7 & 16.3 & 84.7 & 5.5 & 90.7 & \underline{91.0} \\
    Fsh~\citep{li2019faceshifter} & 50.0 & 43.1 & 54.0 & 52.5 & 77.7 & \underline{88.9} & 61.6 & 41.2 & 44.6 & 2.3 & 67.3 & \textbf{92.5} \\
    WDF~\citep{zi2020wilddeepfake} & 35.6 & 63.9 & 56.2 & 60.9 & 84.0 & \underline{85.9} & 63.4 & 21.1 & 63.9 & 6.3 & 82.1 & \textbf{93.0} \\
    ScaleDF~\citep{scaledf} & 22.4 & 73.7 & 44.2 & 53.4 & 76.0 & \underline{83.2} & 74.6 & 55.8 & 73.5 & 81.0 & 82.9 & \textbf{98.6} \\
    MFFI~\citep{miao2025mffi} & 46.1 & 55.2 & 51.0 & 55.8 & 76.5 & \underline{78.6} & 47.8 & 58.1 & 62.6 & 59.2 & 87.4 & \textbf{96.1} \\
    Avg & 36.8 & 57.4 & 53.4 & 52.7 & 87.9 & \underline{88.2} & 62.4 & 40.9 & 68.9 & 13.6 & 74.0 & \textbf{95.8} \\

    \midrule
    \multicolumn{13}{c}{\textbf{AIGC (Accuracy)}} \\
    ForenSynths~\citep{cnnspot} & 48.1 & 57.3 & 57.6 & 57.3 & 49.8 & \underline{74.8} & 68.6 & 71.5 & 71.3 & 69.5 & 77.0 & \textbf{77.2} \\
    DiffusionForensics~\citep{diffusion_detection} & 21.8 & 55.2 & 51.4 & 55.1 & 59.7 & 71.2 & 72.9 & 70.9 & 74.9 & 66.5 & \underline{93.5} & \textbf{99.5} \\
    GenImage~\citep{zhu2023genimage} & 43.8 & 55.1 & 53.4 & 55.0 & 59.0 & 90.5 & 87.8 & 94.3 & \underline{99.0} & 80.9 & 96.3 & \textbf{99.7} \\
    Chameleon~\citep{aide} & 36.7 & 37.9 & 41.2 & 37.8 & 55.2 & 63.1 & 51.6 & 58.9 & 62.9 & 59.6 & \underline{73.2} & \textbf{84.7} \\
    Fakeinversion~\citep{fakeinversion} & 83.8 & 38.4 & 36.7 & 38.3 & 42.3 & \underline{84.6} & 52.4 & 81.2 & 70.0 & 57.6 & 66.7 & \textbf{91.8} \\
    BFree-Online~\citep{bfree} & 36.6 & 67.8 & 60.7 & 67.8 & 38.3 & 55.9 & \underline{71.0} & 32.9 & \textbf{78.6} & 55.2 & 65.5 & 65.7 \\
    SynthWildx~\citep{SynthWildx} & 51.8 & 43.8 & 45.7 & 43.8 & 41.1 & 57.0 & 69.0 & 30.2 & 80.2 & \textbf{83.2} & \underline{81.9} & 80.1 \\
    EvalGEN~\citep{evalgen} & 24.7 & 40.2 & 17.6 & 40.2 & 33.2 & 35.8 & 77.7 & 18.9 & 92.1 & 90.4 & \underline{93.2} & \textbf{96.4} \\
    HydraFake~\citep{veritas} & 54.6 & 49.6 & 51.1 & 49.5 & 69.3 & 62.3 & 62.7 & 60.4 & 77.8 & \underline{87.2} & 71.7 & \textbf{92.8} \\
    Avg & 44.7 & 49.5 & 46.2 & 49.4 & 49.8 & 66.1 & 68.2 & 57.7 & 78.5 & 72.2 & \underline{79.9} & \textbf{87.5} \\

    \midrule
    \multicolumn{13}{c}{\textbf{Doc (Accuracy)}} \\
    DocTamper\_FCD~\citep{qu2023towards} & \underline{73.2} & 73.1 & 68.4 & 64.2 & 52.3 & 60.1 & 77.0 & 38.9 & 1.9 & 39.4 & 25.3 & \textbf{92.8} \\
    DocTamper\_SCD~\citep{qu2023towards} & 69.8 & 58.7 & 67.7 & 53.9 & 39.8 & 26.7 & \underline{71.8} & 24.6 & 1.0 & 31.2 & 25.1 & \textbf{99.8} \\
    DocTamper\_TestingSet~\citep{qu2023towards} & 64.3 & 57.8 & 60.9 & 54.2 & 46.9 & 37.1 & \underline{66.8} & 29.8 & 29.5 & 39.0 & 33.9 & \textbf{99.6} \\
    TextForensicsReasoning~\citep{qu2026textshield} & 43.0 & 51.3 & 51.8 & 52.7 & 51.0 & 50.5 & 52.2 & 46.9 & 52.6 & 52.0 & \underline{54.6} & \textbf{99.6} \\
    Tampered IC13~\citep{wang2022tpic} & \textbf{75.3} & \underline{61.9} & 58.8 & 51.5 & 48.0 & 19.0 & 48.9 & 30.5 & 25.3 & 38.2 & 22.8 & 54.9 \\
    OSTF~\citep{qu2025revisiting} & \underline{60.3} & 47.0 & 59.4 & 51.2 & 57.7 & 55.9 & 57.1 & 57.9 & 57.0 & 56.8 & 58.0 & \textbf{74.9} \\
    RTM~\citep{luo2025rtm} & 45.1 & 51.6 & 59.8 & 47.2 & 47.8 & 38.2 & \underline{63.0} & 33.6 & 32.5 & 42.3 & 33.7 & \textbf{90.0} \\
    % RIFLC~\citep{rific} & 70.5 & 58.1 & \underline{75.4} & 55.9 & 34.4 & 12.8 & \textbf{87.7} & 1.7 & 0.9 & 30.7 & 8.9 & 70.0 \\
    % Avg & 62.6 & 57.4 & 62.7 & 53.8 & 47.2 & 37.5 & \underline{65.5} & 33.0 & 25.1 & 41.2 & 32.9 & \textbf{85.2} \\
    Avg & 61.6 & 57.3 & 61.0 & 53.6 & 49.1 & 41.1 & \underline{62.4} & 37.5 & 28.5 & 42.7 & 36.2 & \textbf{87.4} \\

    \midrule
    \multicolumn{13}{c}{\textbf{Nature (AUC)}} \\
    CASIAv1~\citep{CASIA_2013} & 46.8 & 52.5 & 93.9 & \underline{95.0} & 63.9 & 61.9 & 52.7 & 7.7 & 4.2 & 3.2 & 45.8 & \textbf{96.3} \\
    COVERAGE~\citep{Coverage_2016} & 51.5 & 40.5 & 72.3 & \textbf{76.1} & 53.6 & 49.2 & 52.9 & 50.6 & 50.0 & 0.4 & 55.5 & \underline{75.9} \\
    Columbia~\citep{Columbia_2006} & 62.3 & 2.20 & \underline{99.4} & \textbf{99.8} & 88.0 & 49.2 & 48.2 & 81.7 & 52.6 & 2.5 & 87.6 & 87.7 \\
    NIST16~\citep{NIST16_2019} & 56.0 & 38.7 & 59.4 & 66.5 & 61.6 & 73.4 & \underline{66.7} & 3.9 & 58.7 & 1.2 & 55.4 & \textbf{85.1} \\
    CocoGlide~\citep{trufor2023} & 51.9 & 29.6 & 67.1 & \underline{71.9} & 67.8 & 68.2 & 72.3 & 19.2 & 66.0 & 3.3 & 65.3 & \textbf{76.0} \\
    Autosplice~\citep{jia2023autosplice} & 42.9 & 34.3 & 64.5 & 67.6 & \underline{77.7} & 82.0 & 75.5 & 37.4 & 67.2 & 4.0 & 40.8 & \textbf{99.9} \\
    % IMD2020~\citep{IMD20_2020} & 35.9 & 75.3 & - & - & \textbf{79.3} & 59.4 & 56.5 & 5.9 & 67.2 & 4.0 & 47.8 & \underline{78.0} \\
    OpenSDI~\citep{opensdi} & 35.2 & 42.5 & 57.9 & 57.1 & 52.4 & 77.7 & \underline{84.9} & 5.0 & 73.5 & 1.9 & 69.5 & \textbf{98.6} \\
    DSO-1~\citep{dso-1} & \underline{71.0} & 35.0 & 64.5 & 69.0 & 64.1 & 55.9 & 53.6 & 23.2 & 60.5 & 0.5 & 15.1 & \textbf{82.4} \\
    DEFACTO-12k~\citep{defacto_2019} & 55.1 & 37.8 & \underline{64.3} & 63.9 & 53.6 & 53.5 & 55.3 & 1.7 & 50.0 & 0.9 & 30.9 & \textbf{78.3} \\
    Avg & 52.5 & 34.8 & 71.5 & \underline{74.1} & 64.7 & 63.4 & 62.5 & 25.6 & 53.6 & 2.0 & 51.8 & \textbf{86.7}  \\

    \bottomrule
  \end{tabular}
  }
\end{table}

==> tab/tab_2_mmsec.tex <==
\begin{table}
  \caption{Performance (Accuracy) comparison with baseline methods on OpenMMsec; \textbf{Bold} indicates the best performance; \underline{Underline} indicates the second-best performance.}
  \label{tab:2_mmsec}
  \centering
  \resizebox{0.85\linewidth}{!}{%
  \begin{tabular}{lcccccc}
    \toprule
    \textbf{Method} & \textbf{Venue} & \textbf{DeepFake} & \textbf{AIGC} & \textbf{IMDL} & \textbf{Doc} & \textbf{Avg} \\
    \midrule
    Resnet~\citep{Resnet_2016} & CVPR'16 & 67.8 & 74.2 & 77.3 & 71.7 & 72.7 \\
    EfficientNet~\citep{efficientnet} & ICML'19 & 43.3 & 63.0 & 51.4 & 61.9 & 54.9 \\
    CapsuleNet~\citep{sabour2017dynamic} & NeurIPS'17 & 62.0 & 75.4 & 77.2 &  72.3 & 71.7 \\
    SegFormer~\citep{SegFormer_2021} & NeurIPS'21 & 80.7 & 85.9 & 81.7 & \underline{73.4} & \underline{80.4} \\
    Swin~\citep{Swin_2021} & ICCV'21 & 79.0 & 85.4 & 82.9 & 72.0 & 79.8 \\
    Trufor~\citep{trufor2023} & CVPR'23 & 72.2 & 82.5 & 80.5 & 72.3 & 76.9 \\
    UnivFD~\citep{univfd} & CVPR'23 & 54.2 & 79.8 & 70.9 & 62.7 & 66.9 \\
    Effort~\citep{effort} & ICML'25 & \underline{85.0} & 81.9 & \underline{83.7} & 69.6 & 80.1 \\
    Mesorch~\citep{zhu2025mesorch} & AAAI'25 & 75.7 & 81.4 & 79.9 & 72.7 & 77.4 \\
    CO-SPY~\citep{co-spy} & CVPR'25 & 72.2 & 83.3 & 76.0 & 70.0 & 75.4 \\
    \midrule
    FakeVLM~\citep{fakeclue} & NeurIPS'25 & 75.8 & \underline{86.6} & 66.2 & 14.0 & 60.7 \\
    Veritas~\citep{veritas} & ICLR'26 & 83.4 & 72.8 & 66.8 & 32.1 & 63.8 \\
    FakeShield~\citep{xu2024fakeshield} & ICLR'25 & 72.2 & 73.2 & 59.5 & 68.5 & 68.4 \\
    Ivy-xDetector~\citep{zhang2025ivyfakeunifiedexplainableframework} & Arxiv'25 & 56.3 & 83.1 & 64.2 & 17.7 & 55.3 \\
    \modelbase (Ours) & - & \textbf{89.5} & \textbf{96.4} & \textbf{91.1} & \textbf{90.1} & \textbf{91.8} \\
    %Ours (\modellarge) & - & - & - & - & - & - \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tab/tab_2_seg.tex <==
% \begin{table*}
%   \caption{FIDL Performance comparison (ACC, Img-F1, IoU, Pix-F1.) on benchmarks. All results are averaged.}
%   \label{tab:1_seg}
%   \resizebox{0.975\textwidth}{!}{
%   \begin{tabular}{lcccccccc}
%     \toprule
%         % 第一行表头
%         \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Numbers}} & \multicolumn{4}{c}{\textbf{Small Vision Models}} & \multicolumn{3}{c}{\textbf{FIDL-domain MLLMs}} \\
    
%         \cmidrule(lr){3-6} \cmidrule(lr){7-9} 

%         &  & IML-ViT & MVSS-Net & PSCC-Net & CAT-Net & FakeShield & UniShield & \modelbase \\
%         \midrule
%         \multicolumn{9}{c}{\textbf{IMDL}} \\
%         RTM & - & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- \\
%         CASIA1+ &  - & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- \\
%         \midrule
%         \multicolumn{9}{c}{\textbf{Doc}} \\
%         IMD20 & - & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- \\
%         \midrule
%         \multicolumn{9}{c}{\textbf{Unified FIDL}} \\
%         MMSec$_{ID}$ & - & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- \\
%         MMSec$_{OOD}$ & - & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- & -/-/- \\
%   \bottomrule
%   \end{tabular}
%   }
% \end{table*}

% \begin{table}
%   \caption{Forgery Segment Performance comparison on benchmarks. All results are averaged.}
%   \label{tab:2_seg}
%   \renewcommand{\arraystretch}{0.95} % 将行间距缩小为原来的 0.85 倍
%   \resizebox{0.975\textwidth}{!}{
%   \begin{tabular}{lccccc}
%     \toprule
%         % 第一行表头
% % \multirow{2}{*}{\textbf{Method}} & \multicolumn{10}{c}{\textbf{Small Vision Models}} & \multicolumn{5}{c}{\textbf{FIDL-domain MLLMs}} \\
    
%         % \cmidrule(lr){2-12} \cmidrule(lr){13-16}
        
%         Method & DTD & Mesorch & LEGION & FakeShield & \modelbase \\
%         \midrule
%         \multicolumn{6}{c}{\textbf{Document}} \\
%         DocTamper\_FCD & - & - & - & - & - \\
%         % DocTamper\_SCD & 20.8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         % DocTamper\_TestingSet & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         \midrule
%         \multicolumn{6}{c}{\textbf{Nature}} \\
%         DocTamper\_FCD & - & - & - & - & - \\
%   \bottomrule
%   \end{tabular}
% }
% \end{table}







\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6.5pt}
\caption{Pixel-level forgery localization performance on segmentation benchmarks using binary F1 score (\%). The upper block reports Document benchmarks with document-oriented baselines, and the lower block reports Nature benchmarks with nature-oriented baselines. Unreported results are denoted by ``--''.}
\label{tab:2_seg}
\begin{tabular}{lcccc}
\toprule
\multicolumn{5}{c}{\textbf{Document Benchmarks}} \\
\midrule
Method & DTD & CAFTB & TIFDM & \modelbase \\
\midrule
DocTamperFCD~\citep{qu2023towards}  & {\ul 68.6}    & 29.2       & 9.0  & \textbf{80.8} \\
DocTamperSCD~\citep{qu2023towards}  & {\ul 73.9}    & 37.7       & 25.7 & \textbf{74.9} \\
DocTamperTest~\citep{qu2023towards} & \textbf{80.3} & 32.8       & 25.9 & {\ul 73.3}    \\
T-SROIE~\citep{wang2022tsroie}       & \textbf{92.1} & {\ul 91.7} & 89.4 & 81.7          \\
Tampered IC13~\citep{wang2022tpic} & 83.4          & {\ul 83.9} & 79.7 & \textbf{90.5} \\
OSTF~\citep{qu2025revisiting}          & 56.3          & {\ul 64.8} & 54.1 & \textbf{90.6} \\
RTM~\citep{luo2025rtm}           & 17.2          & {\ul 24.9} & 5.9  & \textbf{59.1} \\
\midrule
Avg           & {\ul 67.4}    & 52.1       & 41.4 & \textbf{78.7} \\
\midrule
\multicolumn{5}{c}{\textbf{Nature Benchmarks}} \\
\midrule
Method & MVSS-Net & TruFor & Mesorch & \modelbase \\
\midrule
CASIAv1~\citep{CASIA_2013}   & 43.5 & 69.2       & \textbf{84.0} & {\ul 78.5}    \\
COVERAGE~\citep{Coverage_2016}  & 45.4 & 52.2       & {\ul 58.6}    & \textbf{71.7} \\
Columbia~\citep{Columbia_2006}  & 78.1 & {\ul 85.9} & \textbf{89.0} & 80.9          \\
NIST16~\citep{NIST16_2019}    & 29.4 & 34.8       & {\ul 39.2}    & \textbf{65.6} \\
CocoGlide~\citep{trufor2023} & {\ul29.1}   & 20.5         & 16.2      & \textbf{62.0} \\
AutoSplice~\citep{jia2023autosplice}& 29.4   & {\ul39.3}         & 24.9      & \textbf{45.7} \\
\midrule
Avg & 42.5 & 50.3 & {\ul52.0} & \textbf{67.4} \\
\bottomrule
\end{tabular}
\end{table*}


==> tab/tab_3_ab1_robust.tex <==
% \begin{table*}[t]
%   \caption{Robust Analysis in Performance (Accuracy) comparison with baseline methods on OpenMMsec.}
%   \label{tab:3_robust}
%   \centering
%   \resizebox{0.95\linewidth}{!}{%
%   \begin{tabular}{lc|cccc|cccc|cc|cc|cc|cc|cc}
%     \toprule
%     \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Original}} 
%     & \multicolumn{4}{c|}{\textbf{JPEG Compression (QF)}} 
%     & \multicolumn{4}{c|}{\textbf{Gaussian Blur ($\sigma$)}} 
%     & \multicolumn{2}{c|}{\textbf{Resize}} 
%     & \multicolumn{2}{c|}{\textbf{Noise}} 
%     & \multicolumn{2}{c|}{\textbf{Brightness}} 
%     & \multicolumn{2}{c|}{\textbf{Saturation}} 
%     & \multicolumn{2}{c}{\textbf{Contrast}} \\
%     & & 95 & 90 & 75 & 50 
%     & 1.0 & 2.0 & 3.0 & 4.0 
%     & 0.5 & 2.0 
%     & 10 & 20 
%     & 0.5 & 1.5 
%     & 0.5 & 1.5 
%     & 0.5 & 1.5 \\ 
%     \midrule
%     DTD      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     FFDN     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     TruFor   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     Mesorch  & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     CDFA     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     Effort   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     AIDE     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     DRCT     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     DDA      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     Mirror   & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \textbf{\baseline} & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \bottomrule
%   \end{tabular}%
%   }
% \end{table*}



\begin{table}[!t]
\caption{
Average robustness analysis on OpenMMsec~\citep{du2026SICA}. 
This table only reports the averaged results over perturbation strengths, while the complete robustness table is provided in Table~\ref{tab:3_robust_full}.
}
  \label{tab:3_robust}
  \centering
  \resizebox{0.95\linewidth}{!}{%
  \begin{tabular}{l|ccccccc}
    \toprule
    \textbf{Perturbation} 
    & \textbf{FFDN} 
    & \textbf{Mesorch} 
    & \textbf{Effort} 
    & \textbf{ForensicsAdapter} 
    & \textbf{ForensicMOE} 
    & \textbf{FakeShield} 
    & \textbf{\modelbase} \\
    \midrule
    Gaussian Blur    & 47.63 & 49.45 & 56.71 & 55.76 & 54.11 & 64.63 & \textbf{79.46} \\
    Brightness       & 44.78 & 51.06 & 57.53 & 56.10 & 54.82 & 63.48 & \textbf{70.60} \\
    Contrast         & 43.65 & 51.12 & 58.27 & 56.22 & 55.53 & 63.86 & \textbf{76.26} \\
    JPEG Compression & 39.93 & 52.00 & 58.73 & 56.78 & 51.67 & 62.77 & \textbf{76.16} \\
    Noise            & 48.03 & 48.18 & 54.62 & 52.77 & 53.62 & 63.54 & \textbf{65.32} \\
    Resize           & 44.19 & 50.54 & 58.69 & 57.02 & 53.47 & 51.30 & \textbf{69.23} \\
    Saturation       & 40.69 & 51.69 & 58.43 & 57.30 & 55.77 & 64.30 & \textbf{81.85} \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tab/tab_4_ab2_quality.tex <==
\begin{table}
  \caption{Robust Analysis in Performance (Accuracy) comparison with baseline methods on OpenMMsec.}
  \label{tab:4_robust}
  \centering
  \resizebox{0.85\linewidth}{!}{%
  \begin{tabular}{lc|cccc|cccc|cc|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Original}} & \multicolumn{4}{c|}{\textbf{JPEG Compression (QF)}} & \multicolumn{4}{c|}{\textbf{Gaussian Blur ($\sigma$)}} & \multicolumn{2}{c|}{\textbf{Resize}} & \multicolumn{2}{c|}{\textbf{Noise}} & \multicolumn{2}{c|}{\textbf{Brightness}} & \multicolumn{2}{c|}{\textbf{Saturation}} & \multicolumn{2}{c}{\textbf{Contrast}} \\
    & & 95 & 90 & 75 & 50 & 1.0 & 2.0 & 3.0 & 4.0 & 0.5 & 2.0 & 10 & 20 & 0.5 & 1.5 & 0.5 & 1.5 & 0.5 & 1.5 \\ 
    \midrule
    \textbf{\baseline} & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
    \bottomrule
  \end{tabular}
    }
\end{table}

==> tab/tab_5_tts.tex <==
\begin{table*}
  \caption{Impact of decoding hyperparameters on OpenMMsec. Left: different random seeds. Right: different sampling temperatures.}
  \label{tab:5_tts}
  \centering
  % \resizebox{0.85\linewidth}{!}{%
\begin{tabular}{c|cc @{\hspace{1.5em}} c|cc}
\toprule
\multicolumn{3}{c}{\textbf{(a) Seed}} & \multicolumn{3}{c}{\textbf{(b) Temperature}} \\
\cmidrule(r){1-3} \cmidrule(l){4-6}
Seed & ACC & F1 & Temp & ACC & F1 \\
\midrule
42    & 91.8 & 93.4 & 0.1 & 91.8 & 93.4 \\
1024   & 91.7 & 93.5 & 0.5 & 91.8 & 92.5 \\
8192 & 91.8 & 93.5 & 0.9 & 91.7 & 93.5 \\
\bottomrule
\end{tabular}
    % }
\end{table*}

==> tab/tab_ab_domain.tex <==
\begin{table}[t]
\begin{minipage}{0.56\textwidth}
\centering
\captionof{table}{Ablation Study on Forensic Domains and Tasks.}
\label{tab:single_vs_multi_domain}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Doc} & \textbf{IMDL} & \textbf{Deepfake} & \textbf{AIGC} & \textbf{Avg.} \\
\midrule
DeFakerOne (stage3. Multi-Task) & \textbf{92.5} & \underline{89.7} & \underline{89.0} & \textbf{96.8} & \textbf{92.0} \\
\midrule
DeFakerOne (stage2. Data-Scaling) & \underline{90.1} & \textbf{91.1} & \textbf{89.5} & \underline{96.4} & \underline{91.8} \\
\midrule
DeFakerOne (stage1. Multi-Domain) & 89.7 & 54.5 & 77.4 & 85.9 & 76.8 \\
\midrule
Nature Specialized   & 66.6 & 74.6 & 64.3 & 74.5 & 70.0 \\
AIGC Specialized     & 13.9 & 53.2 & 28.3 & 92.9 & 47.1 \\
Deepfake Specialized & 13.8 & 47.6 & 88.7 & 45.8 & 49.0  \\
Doc Specialized      & 89.5 & 55.5 & 29.2 & 44.3 & 54.6 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.40\textwidth}
\centering
\captionof{table}{Decoding hyperparameters.}
\label{tab:5_tts}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc @{\hspace{1.2em}} c|cc}
\toprule
\multicolumn{3}{c}{\textbf{(a) Seed}} & \multicolumn{3}{c}{\textbf{(b) Temperature}} \\
\cmidrule(r){1-3} \cmidrule(l){4-6}
\textbf{Seed} & \textbf{ACC} & \textbf{F1} & \textbf{Temp} & \textbf{ACC} & \textbf{F1} \\
\midrule
42   & 91.8 & 93.4 & 0.1 & 91.8 & 93.4 \\
1024 & 91.7 & 93.5 & 0.5 & 91.8 & 92.5 \\
8192 & 91.8 & 93.5 & 0.9 & 91.7 & 93.5 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}

==> tab/tab_dataset_consist.tex <==
\begin{table*}[t]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{llcccc}
\toprule
Domain & Total & Dataset/Size & Dataset/Size & Dataset/Size & Dataset/Size \\
\midrule

\multirow{3}{*}{DeepFake} 
& \multirow{3}{*}{3.1M}
& \makecell{FF++~\citep{rossler2019faceforensics++}\\0.11M}
& \makecell{CelebDF-v2~\citep{li2020celeb}\\0.18M}
& \makecell{DFD~\citep{dfd2019}\\0.10M}
& \makecell{DFDC~\citep{dfd2019}\\0.09M} \\
& 
& \makecell{ScaleDF~\citep{scaledf}{}\\0.14M}
& \makecell{DF40~\citep{yan2024df40}\\0.10M}
& \makecell{WDF~\citep{zi2020wilddeepfake}\\0.10M}
& \makecell{MFFI~\citep{miao2025mffi}\\0.06M} \\
& 
& \makecell{Private Dataset\\2.22M}
& --
& --
& -- \\
\midrule

\multirow{2}{*}{AIGC}
& \multirow{2}{*}{3.6M}
& \makecell{DiffusionForensics~\citep{dire}\\0.034M}
& \makecell{CommunityForensics~\citep{CommunityForensics}\\0.95M}
& \makecell{GenImage~\citep{zhu2023genimage}\\0.09M}
& \makecell{LAION\_DATA~\citep{schuhmann2022laion}\\1.20M} \\
&
& \makecell{ForenSynths~\citep{cnnspot}\\0.07M}
& \makecell{Private Dataset\\1.256M}
& --
& -- \\
\midrule

\multirow{2}{*}{Document}
& \multirow{2}{*}{2.5M}
& \makecell{DocTamper~\citep{qu2023towards}\\0.145M}
& \makecell{T-SROIE~\citep{wang2022tsroie}\\0.0006M}
& \makecell{RTM~\citep{luo2025rtm}\\0.009M}
& \makecell{SACP~\citep{sacp}\\0.003M} \\
&
& \makecell{RIFLC~\citep{rific}\\0.002M}
& \makecell{OSTF~\citep{qu2025revisiting}\\0.0022M}
& \makecell{Private Dataset\\2.338M}
& -- \\
\midrule

\multirow{2}{*}{Nature}
& \multirow{2}{*}{3.3M}
& \makecell{MIML~\citep{qu2024towards}\\0.937M}
& \makecell{CASIA-v2~\citep{CASIA_2013}\\0.06M}
& \makecell{COCO\_2017~\citep{mscoco_2014}\\0.82M}
& \makecell{OpenSDI~\citep{opensdi}\\0.20M} \\
&
& \makecell{So-Fake-OOD~\citep{huang2025sofakebenchmarkingexplainingsocial}\\0.062M}
& \makecell{So-Fake-Set~\citep{huang2025sofakebenchmarkingexplainingsocial}\\1.20M}
& --
& -- \\

\bottomrule
\end{tabular}
}
\caption{Composition of the DeFakerOne training data.}
\label{tab:training_data_composition}
\end{table*}


==> tab/tab_robust_full.tex <==
\begin{table}[!t]
  \caption{Robust analysis (Accuracy) comparison with baseline methods on OpenMMsec~\citep{du2026SICA}.}
  \label{tab:3_robust_full}
  \centering
  \resizebox{0.95\linewidth}{!}{%
  \begin{tabular}{ll|ccccccc}
    \toprule
    \multicolumn{2}{c}{\textbf{Method}} 
    & \textbf{FFDN} 
    & \textbf{Mesorch} 
    & \textbf{Effort} 
    & \textbf{ForensicsAdapter} 
    & \textbf{ForensicMOE} 
    & \textbf{FakeShield} 
    & \textbf{\modelbase} \\
    \midrule
    \multirow{6}{*}{Gaussian Blur}
    & 0.5 & 42.84 & 51.78 & 59.30 & 57.65 & 55.70 & 62.86 & \textbf{85.44} \\
    & 1.0 & 46.32 & 50.43 & 58.43 & 56.70 & 55.13 & 63.46 & \textbf{80.72} \\
    & 1.5 & 48.68 & 49.07 & 56.55 & 55.75 & 53.63 & 65.57 & \textbf{77.59} \\
    & 2.0 & 49.68 & 48.67 & 55.23 & 54.95 & 53.13 & 65.54 & \textbf{76.81} \\
    & 2.5 & 50.62 & 47.30 & 54.03 & 53.77 & 52.95 & 65.74 & \textbf{76.74} \\
    & Avg & 47.63 & 49.45 & 56.71 & 55.76 & 54.11 & 64.63 & \textbf{79.46} \\
    \midrule
    \multirow{6}{*}{Brightness}
    & 0.5 & 44.65 & 53.00 & 57.88 & 56.17 & 55.35 & 64.01 & \textbf{81.44} \\
    & 1.0 & 39.68 & 51.58 & 58.90 & 57.75 & 55.70 & 63.14 & \textbf{84.59} \\
    & 1.5 & 44.59 & 50.80 & 58.75 & 57.15 & 55.33 & 64.34 & 50.33 \\
    & 2.0 & 46.78 & 50.03 & 57.15 & 55.67 & 54.15 & 63.61 & \textbf{70.36} \\
    & 2.5 & 48.22 & 49.87 & 54.95 & 53.80 & 53.58 & 62.31 & \textbf{66.26} \\
    & Avg & 44.78 & 51.06 & 57.53 & 56.10 & 54.82 & 63.48 & \textbf{70.60} \\
    \midrule
    \multirow{6}{*}{Contrast}
    & 0.5 & 44.61 & 52.28 & 58.58 & 56.00 & 55.03 & 63.41 & \textbf{80.97} \\
    & 1.0 & 39.68 & 51.58 & 58.90 & 57.75 & 55.70 & 64.69 & \textbf{84.52} \\
    & 1.5 & 43.38 & 50.80 & 59.05 & 56.70 & 56.10 & 64.31 & \textbf{76.24} \\
    & 2.0 & 44.88 & 50.45 & 57.40 & 55.97 & 55.50 & 64.31 & \textbf{71.06} \\
    & 2.5 & 45.68 & 50.50 & 57.43 & 54.72 & 55.30 & 62.76 & \textbf{68.51} \\
    & Avg & 43.65 & 51.12 & 58.27 & 56.22 & 55.53 & 63.86 & \textbf{76.26} \\
    \midrule
    \multirow{6}{*}{JPEG Compression}
    & 75 & 39.95 & 51.78 & 58.68 & 56.67 & 51.35 & 62.94 & \textbf{78.36} \\
    & 80 & 39.58 & 52.30 & 58.75 & 56.95 & 50.88 & 62.69 & \textbf{76.59} \\
    & 85 & 39.38 & 52.00 & 57.13 & 56.37 & 51.25 & 63.46 & \textbf{75.29} \\
    & 90 & 40.75 & 51.63 & 59.58 & 56.80 & 51.55 & 62.01 & \textbf{75.04} \\
    & 95 & 40.01 & 52.25 & 59.53 & 57.15 & 53.33 & 62.74 & \textbf{75.51} \\
    & Avg & 39.93 & 52.00 & 58.73 & 56.78 & 51.67 & 62.77 & \textbf{76.16} \\
    \midrule
    \multirow{6}{*}{Noise}
    & 0.05 & 45.28 & 47.82 & 57.28 & 55.20 & 53.68 & 63.66 & \textbf{71.66} \\
    & 0.1 & 47.88 & 47.42 & 55.53 & 52.52 & 55.95 & 63.66 & \textbf{64.83} \\
    & 0.15 & 47.58 & 47.37 & 54.58 & 52.50 & 54.10 & 63.26 & \textbf{61.23} \\
    & 0.2 & 48.98 & 48.27 & 53.30 & 52.15 & 52.70 & 63.54 & 63.36 \\
    & 0.25 & 50.42 & 50.00 & 52.50 & 51.50 & 51.68 & 63.59 & \textbf{65.53} \\
    & Avg & 48.03 & 48.18 & 54.62 & 52.77 & 53.62 & 63.54 & \textbf{65.32} \\
    \midrule
    \multirow{6}{*}{Resize}
    & 128 & 49.48 & 50.53 & 57.18 & 54.02 & 52.50 & 52.13 & \textbf{61.21} \\
    & 256 & 45.32 & 49.32 & 58.43 & 57.25 & 54.15 & 50.85 & \textbf{69.21} \\
    & 384 & 43.18 & 50.18 & 59.55 & 58.20 & 53.90 & 50.73 & \textbf{71.14} \\
    & 512 & 40.51 & 50.98 & 59.55 & 58.17 & 53.68 & 51.35 & \textbf{70.29} \\
    & 640 & 42.48 & 51.70 & 58.75 & 57.50 & 53.10 & 51.43 & \textbf{74.32} \\
    & Avg & 44.19 & 50.54 & 58.69 & 57.02 & 53.47 & 51.30 & \textbf{69.23} \\
    \midrule
    \multirow{6}{*}{Saturation}
    & 0.5 & 40.75 & 52.38 & 58.93 & 57.25 & 54.95 & 64.69 & \textbf{82.24} \\
    & 1.0 & 39.68 & 51.58 & 58.90 & 57.75 & 55.70 & 63.74 & \textbf{84.57} \\
    & 1.5 & 39.95 & 51.65 & 58.50 & 57.05 & 56.10 & 64.69 & \textbf{83.17} \\
    & 2.0 & 40.95 & 51.23 & 58.08 & 57.37 & 55.58 & 64.56 & \textbf{80.79} \\
    & 2.5 & 42.11 & 51.60 & 57.73 & 57.10 & 56.53 & 64.01 & \textbf{78.49} \\
    & Avg & 40.69 & 51.69 & 58.43 & 57.30 & 55.77 & 64.30 & \textbf{81.85} \\
    \bottomrule
  \end{tabular}
  }
\end{table}
